Numerical study of viscous starting flow past a flat plate

Viscous flow past a finite plate which is impulsively started in direction normal to itself is studied numerically using a high order mixed finite difference and semi-Lagrangian scheme. The goal is to resolve details of the vorticity generation at early times, and to determine the effect of viscosity on flow quantities such as the core trajectory and vorticity, and the shed circulation. Vorticity contours, streaklines and streamlines are presented for a range of Reynolds numbers $Re \in [250, 2000]$ and a range of times $t \in[0. 0002, 5]$. At early times, most of the vorticity is attached to the plate. The paper proposes a definition for the shed circulation at early as well as late times, and shows that it indeed represents vorticity that separates from the plate without reattaching. The contribution of viscous diffusion to the circulation shedding rate is found to be significant, but, interestingly, to depend only slightly on the value of the Reynolds number. The shed circulation and the vortex core trajectories follow scaling laws for inviscid self-similar flow over several decades in time. Scaling laws describing the core vorticity, core dissipation, boundary layer thickness, drag and lift forces in time and Reynolds number are also presented. The simulations provide benchmark results to evaluate, for example, simpler separation models such as point vortex and vortex sheet models.

==> sec05_conc.tex <==
\section{Summary}
\label{sec:conc}
Viscous flow past a flat plate of
zero thickness which
is impulsively started in direction normal to itself is studied using
highly resolved numerical simulations.
The main features of the flow revealed by the computations are the following.
%Viscous flow past a flat plate impulsively started in direction 
%normal to itself was computed using a time-splitting method 
%based on fourth order finite differences on a regular mesh 
%of a rectangular domain.
%Convection is computed using a semi-Lagrange method,
%and diffusion is computed using the implicit Crank-Nicholson method.
%The main contributions are 
%to reveal detailed aspects of the flow and its dependence on Re

\renewcommand{\labelenumi}{(\arabic{enumi})}
\begin{enumerate}[(1)]
\item
Detailed features of the early starting flow are documented,
such as 
the growth of the leading vortex emanating from the boundary layer,
the growth of the region of opposite-signed vorticity on the plate,
and 
the evolution of the plate vorticity and vorticity gradients.

\item
The effect of Reynolds numbers $Re\in[250,2000]$
on the vorticity and dissipation fields, and on the
shape of particle streakline is described. 
including thinning of boundary layer and shear layer thicknesses,
tightening of the spiral streakline turns in the vortex center.
and increasing core vorticities and dissipation.

%\item
Scaling behaviours are observed
for several quantities in the flow
over several decades in time.
They capture the dependence on time and on the Reynolds number.
Some quantities clearly depend strongly on $Re$, such as
the core vorticity, the boundary layer thickness, and the lift over the half-plate, with
\begin{eqnarray*}
%\text{core vorticity}
 \omega_c(t)&\approx& 0.335 Re^{3\over4}t^{-{3\over 4}}~,\\%\quad\text{ as } t\to 0\\
%\text{boundary layer thickness}& 
\delta(t)&\sim& t^{1\over2}Re^{-{1\over2}}~,\\%\quad\text{ as } t\to 0\\
%\text{drag} & &
F_L(t)&\approx& Re^{-{1\over2}} t^{-{1\over2}}~,
\end{eqnarray*}
as $t\to 0$.
Other quantities of the early starting flow 
are largely independent on $Re$, such as
the core trajectory, the shed circulation, the size of the recirculation region,
and the lift force, with well resolved scalings obtained for,
\begin{eqnarray*}
y_c(t)&\approx& 0.37 t^{2/3}~,\\% \quad\text{ as } t\to 0\\
x_c(t)-0.5&\approx& -0.1t^{2/3}~,\\% \quad\text{ as } t\to 0\\
\Gamma(t)&\approx& 2t^{1/3}~,% \quad\text{ as } t\to 0
%\text{recirculation region size}&  &s(t)\quad \text{(no scaling)}\\
%\text{total negative vorticity}&  &\Gamma_N(t)\quad \text{(no scaling)}\\
%\text{lift} & &F_L(t) \quad \text{(mild dependence on Re)} \sim t^{\alpha}
\end{eqnarray*}
all as $t\to 0$.

%\item
%Circulation definition, 
%scaling over various decades
%viscous contribution to flux due to diffusion across boundaries near tip 
%large, but largely independent of Re
We
compute the shed circulation, as well as circulation shedding
rates across various components of the boundary of the leading vortex.
We find that

The shed circulation satisfies the self-similar scaling
laws over more than 3 decades.

The largest component of the circulation shedding
rate is convection of vorticity below the plate into the
leading vortex. This component is strikingly independent of
the Reynolds number.

The next largest component, in magnitude, is the flux
out
of the region that defines the leading vortex due to diffusion across the lower boundary
above the plate. This component also appears to not
depend on $Re$ at early times.
In view of equation (4),
this suggests that gradients of vorticity grow like $Re$.
The resulting total circulation depends very little on Re.

Almost no vorticity flows through the slant boundary
of the vortex, as defined in figure 2, showing that it
separates vorticity in the leading vortex from attached
boundary layer vorticity.

\end{enumerate}


In summary, the main contributions are 
to resolve detailed aspects over several decades,
including accurate computation of viscous circulation and shedding rates,
that provide benchmark results that can be used to
evaluate simpler vortex shedding models.
A comparison with a vortex sheet separation model will be presented elsewhere.

